Interpretation of Emergent Communication in Heterogeneous Collaborative Embodied Agents

Communication between embodied AI agents has received increasing attention in recent years. Despite its use, it is still unclear whether the learned communication is interpretable and grounded in perception. To study the grounding of emergent forms of communication, we first introduce the collaborative multi-object navigation task CoMON. In this task, an oracle agent has detailed environment information in the form of a map. It communicates with a navigator agent that perceives the environment visually and is tasked to find a sequence of goals. To succeed at the task, effective communication is essential. CoMON hence serves as a basis to study different communication mechanisms between heterogeneous agents, that is, agents with different capabilities and roles. We study two common communication mechanisms and analyze their communication patterns through an egocentric and spatial lens. We show that the emergent communication can be grounded to the agent observations and the spatial structure of the 3D environment. Video summary: https://youtu.be/kLv2rxO9t0g

==> sections/fig/1ON_vs_2ON_Dcomm.tex <==
\begin{figure*}
\resizebox{\linewidth}{!}{
\newcolumntype{C}{>{\centering\arraybackslash} m{8.8cm} }
\newcolumntype{D}{>{\centering\arraybackslash} m{1cm} }
\begin{tabular}{@{}DCCCC@{}}
    \rotatebox{90}{\LARGE{\mon{1}}} &
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_1ON_m_O_to_N_exploded_0_new.pdf} &  
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_1ON_m_O_to_N_exploded_1_new.pdf} &  
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_1ON_m_O_to_N_exploded_2_new.pdf} &  
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_1ON_m_O_to_N_new.pdf}\\
    \rotatebox{90}{\LARGE{\mon{2} Distinguishable goals}} &
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_2ON_m_O_to_N_exploded_distinguishable_0.pdf} &  
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_2ON_m_O_to_N_exploded_distinguishable_1.pdf} &  
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_2ON_m_O_to_N_exploded_distinguishable_2.pdf} &  
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_2ON_m_O_to_N_distinguishable.pdf}   \\
    \rotatebox{90}{\LARGE{\mon{2} Indistinguishable Goals}} &
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_2ON_m_O_to_N_exploded_indistinguishable_0.pdf} &  
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_2ON_m_O_to_N_exploded_indistinguishable_1.pdf} &  
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_2ON_m_O_to_N_exploded_indistinguishable_2.pdf} &  
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_2ON_m_O_to_N_indistinguishable.pdf}   
\end{tabular}
}
\caption{
\textbf{Egocentric visualization of \DiscCom communication symbol $m_{O \rightarrow N}^2$}. First row is for \mon{1}, second row is for \mon{2} distinguishable goals, third row is for \mon{2} indistinguishable goals.
}
\label{fig:disc_com_1vs2ON}
\end{figure*}






==> sections/fig/1ON_vs_2ON_Ucomm.tex <==
\begin{figure*}
\resizebox{\linewidth}{!}{
\newcolumntype{C}{>{\centering\arraybackslash} m{8.8cm} }
\begin{tabular}{@{}CC@{}}
{$1^{st}$ element} & {$2^{nd}$ element} \\
    \includegraphics[width=1\linewidth]{plots/cont_comm_length2_1ON_m_O_to_N_round_1_0_new.pdf}
    &
    \includegraphics[width=1\linewidth]{plots/cont_comm_length2_1ON_m_O_to_N_round_1_1_new.pdf}\\
    \includegraphics[width=1\linewidth]{plots/cont_comm_length2_2ON_m_O_to_N_round_1_0.pdf}
    &
    \includegraphics[width=1\linewidth]{plots/cont_comm_length2_2ON_m_O_to_N_round_1_1.pdf}
\end{tabular}
}
\caption{
\textbf{Egocentric visualization of \ContCom communication symbol $m_{O \rightarrow N}^2$.} First row is for \mon{1} and second row is for \mon{2}.
}
\label{fig:cont_com_1vs2ON}
\end{figure*}






==> sections/fig/cont_comm_2ON_m_O_to_N_round0.tex <==
\begin{figure*}
\resizebox{\linewidth}{!}{
\newcolumntype{C}{>{\centering\arraybackslash} m{8.8cm} }
\begin{tabular}{@{}CC@{}}
{$1^{st}$ element} & {$2^{nd}$ element} \\
    \includegraphics[width=1\linewidth]{plots/cont_comm_length2_2ON_m_O_to_N_round_0_0.pdf}
    &
    \includegraphics[width=1\linewidth]{plots/cont_comm_length2_2ON_m_O_to_N_round_0_1.pdf}
\end{tabular}
}
\caption{
\textbf{Egocentric visualization of \ContCom communication symbol} $m_{O \rightarrow N}^1$ \textbf{for \mon{2}.}
The two plots visualize the value of the first and second element of the message plotted \wrt the relative coordinates of the goal object from \atwo.
The navigator agent \atwo is facing the +y axis and its field-of-view is marked with red lines.
The plot on the left corresponds to the $1^\text{st}$ dimension of the message, while the plot on the right corresponds to the $2^\text{nd}$ dimension.
The value of each dimension is indicated by the color hue.
}
\label{fig:cont_comm_2ONm_O_to_N_round_0}
\end{figure*}




==> sections/fig/cont_comm_len2_action_distribution.tex <==
\begin{figure}
\centering
\includegraphics[width=0.45\textwidth]{plots/cont_comm_len2_action_distribution.pdf}
\caption{
\textbf{Value of first and second element of $m_{O \rightarrow N}^2$ vs action in \ContCom.}
\SP{No strong conclusions can be drawn. This is intuitive. $m_{O \rightarrow N}^2$ encodes the \textit{long-term goal} which need not be correlated with the next action.}
\todo{If there is no conclusion to convey here, remove this figure.}
}
\label{fig:cont_comm_len2_action_distribution}
\end{figure}


==> sections/fig/disc_comm_2ON_vocab2_m_O_to_N_distinguishable_round0.tex <==
\begin{figure*}
\resizebox{\linewidth}{!}{
\newcolumntype{C}{>{\centering\arraybackslash} m{8.8cm} }
\begin{tabular}{@{}CCCC@{}}
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_2ON_m_O_to_N_exploded_distinguishable_0_round0.pdf} &  
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_2ON_m_O_to_N_exploded_distinguishable_1_round0.pdf} &  
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_2ON_m_O_to_N_exploded_distinguishable_2_round0.pdf} &  
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_2ON_m_O_to_N_distinguishable_round0.pdf}   
\end{tabular}
}
\caption{
\textbf{Egocentric visualization of \DiscCom communication symbol $m_{O \rightarrow N}^2$ when the goals are distinguishable by \aone.}
The plots show the relative coordinates of the current goal object from \atwo's perspective when \aone communicates the symbol through \DiscCom with vocabulary size two.
The navigator agent (\atwo) is facing the +y axis and its field-of-view is marked with red lines.
Data points are accumulated across all validation episodes, and we plot contour lines of the bivariate density distribution.
Each data point is a message with $(x,y)$ coordinates determined from the coordinates of the current goal object in \atwo's egocentric reference frame when the message was sent.
The first three plots are for each communication symbol, and the right-most combines all symbols.
Note how each symbol represents distinct regions that are egocentrically organized around the agent: \symone captures `behind and not visible', \symtwo corresponds mostly to `close, in front', and \symthree is `farther in front'.
}
\label{fig:disc_comm_2ON_m_O_to_N_distinguishable_round0}
\end{figure*}






==> sections/fig/disc_comm_2ON_vocab2_m_O_to_N_indistinguishable.tex <==
\begin{figure*}
\resizebox{\linewidth}{!}{
\newcolumntype{C}{>{\centering\arraybackslash} m{8.8cm} }
\begin{tabular}{@{}CCCC@{}}
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_2ON_m_O_to_N_exploded_indistinguishable_0.pdf} &  
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_2ON_m_O_to_N_exploded_indistinguishable_1.pdf} &  
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_2ON_m_O_to_N_exploded_indistinguishable_2.pdf} &  
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_2ON_m_O_to_N_indistinguishable.pdf}   
\end{tabular}
}
\caption{
\textbf{Egocentric visualization of \DiscCom communication symbol $m_{O \rightarrow N}^2$ when the goals are indistinguishable by \aone.}
The plots show the relative coordinates of the current goal object from \atwo's perspective when \aone communicates the symbol through \DiscCom with vocabulary size two.
The navigator agent (\atwo) is facing the +y axis and its field-of-view is marked with red lines.
Data points are accumulated across all validation episodes, and we plot contour lines of the bivariate density distribution.
Each data point is a message with $(x,y)$ coordinates determined from the coordinates of the current goal object in \atwo's egocentric reference frame when the message was sent.
The first three plots are for each communication symbol, and the right-most combines all symbols.
Note how each symbol represents distinct regions that are egocentrically organized around the agent: \symone captures `behind and not visible', \symtwo corresponds mostly to `close, in front', and \symthree is `farther in front'.
}
\label{fig:disc_comm_2ON_m_O_to_N_indistinguishable}
\end{figure*}






==> sections/fig/disc_comm_2ON_vocab2_m_O_to_N_indistinguishable_round0.tex <==
\begin{figure*}
\resizebox{\linewidth}{!}{
\newcolumntype{C}{>{\centering\arraybackslash} m{8.8cm} }
\begin{tabular}{@{}CCCC@{}}
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_2ON_m_O_to_N_exploded_indistinguishable_0_round0.pdf} &  
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_2ON_m_O_to_N_exploded_indistinguishable_1_round0.pdf} &  
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_2ON_m_O_to_N_exploded_indistinguishable_2_round0.pdf} &  
    \includegraphics[width=1\linewidth]{plots/disc_comm_vocab2_2ON_m_O_to_N_indistinguishable_round0.pdf}   
\end{tabular}
}
\caption{
\textbf{Egocentric visualization of \DiscCom communication symbol $m_{O \rightarrow N}^1$ when the goals are indistinguishable by \aone.}
The plots show the relative coordinates of the current goal object from \atwo's perspective when \aone communicates the symbol through \DiscCom with vocabulary size two.
The navigator agent (\atwo) is facing the +y axis and its field-of-view is marked with red lines.
Data points are accumulated across all validation episodes, and we plot contour lines of the bivariate density distribution.
Each data point is a message with $(x,y)$ coordinates determined from the coordinates of the current goal object in \atwo's egocentric reference frame when the message was sent.
The first three plots are for each communication symbol, and the right-most combines all symbols.
Note how each symbol represents distinct regions that are egocentrically organized around the agent: \symone captures `behind and not visible', \symtwo corresponds mostly to `close, in front', and \symthree is `farther in front'.
}
\label{fig:disc_comm_2ON_m_O_to_N_indistinguishable_round0}
\end{figure*}





